Facial Action Unit Detection using 3D Facial Landmarks

In this paper, we propose to detect facial action units (AU) using 3D facial landmarks. Specifically, we train a 2D convolutional neural network (CNN) on 3D facial landmarks, tracked using a shape index-based statistical shape model, for binary and multi-class AU detection. We show that the proposed approach is able to accurately model AU occurrences, as the movement of the facial landmarks corresponds directly to the movement of the AUs. By training a CNN on 3D landmarks, we can achieve accurate AU detection on two state-of-the-art emotion datasets, namely BP4D and BP4D+. Using the proposed method, we detect multiple AUs on over 330,000 frames, reporting improved results over state-of-the-art methods.

==> experiments.tex <==
\section{Experiments}
\label{sec:Exp}
\subsection{Facial expression databases}
\label{sec:DB}
\textbf{BP4D} was used in the Facial Expression Recognition and Analysis (FERA) challenge in 2015  \cite{valstarFERA15} and 2017 \cite{valstarFERA17}; containing 2D and 3D data. It contains 41 subjects with eight dynamic expressions plus neutral. The dataset contains 18 male and 23 female subjects ages 18-29 years of age, with a range of ethnicities. For each sequence in this database, approximately 500 frames contain AU occurrences; we used all labeled frames, which is over 140,000.\\
\textbf{BP4D+} consists of 140 subjects (58 males and 82 females); ages 18-66, each with highly varied emotional responses. It includes thermal, physiological, 2D, and 3D data. It was also used in the FERA challenge 2017 \cite{valstarFERA17}. Like BP4D, approximately 500 frames per sequence contain AU occurrences; we used all labeled frames which is over 190,000.

\subsection{Experimental Design}
\label{sec:expDesign}
We detected 83 3D facial landmarks on all AU labeled frames from BP4D and BP4D+, using a shape-index-based statistical shape model \cite{canavan2015landmark}. We then normalized the 83 landmarks to [0,23] ($C=24$). While any number of landmarks that represent a face with AU occurrences can be used, we chose 83 to be consistent with other related works \cite{zhang2016multimodal}, \cite{zhang2014bp4d}, \cite{valstarFERA17}, \cite{fabiano2018}. We then transform the normalized landmarks to a binary representation in a 3 dimensional array of $24 \times 24 \times 24$ (Figure \ref{fig:overview} (d)).

We consider both binary \cite{li2017action} and 3-class \cite{chu2017learning} classification. For binary classification, the presence/absence of an action unit was coded as 1/0. For the 3-class classification, the presence/absence of an action unit was coded as 1/-1 and 0 when no information was available \cite{chu2017learning}. 

For the binary-class, our CNN consists of 8 layers; two convolutional layers followed by a max pooling layer, two more convolutional layers, another max pooling layer and finally three fully connected layers. The output layer has 12 binary outputs for the 12 AUs being predicted. The activation function for each of the hidden layers is relu \cite{jarrett2009best} and the activation function for the output layer is sigmoid \cite{han1995influence}, the loss function for this network was binary cross-entropy and the optimizer used was adam \cite{kingma2014adam} (Figure \ref{fig:overview}). All training is done with 250 epochs.

For the 3-class, we use a similar network with common convolutional
layers, but different fully connected layers for each AU (a common output layer can not predict the 3-classes for all the AUs). The loss function was categorical cross-entropy and the activation function for the initial layers was still relu, but for the output layers it was softmax \cite{bridle1990probabilistic}, as it  performs well for multi-class classification \cite{duan2003multi}. Again, all training is done with 250 epochs.

For binary-class, we used 3-fold and 10-fold cross-validation, for 3-class problem we used 3-fold cross-validation. We also balanced the distribution of positive and negative samples (i.e. occurrence of AUs), as the distribution of AUs is not consistent (Table \ref{Distribution}). We chose this experimental design to be consistent with related works \cite{chu2017learning}, \cite{li2017action}. As can be seen from Table \ref{Distribution}, some of the AUs have a small number of frames where the AU occurred, especially in BP4D+.
\begin{table}
\centering
\captionsetup{justification=centering}
 \begin{tabular}{|p{0.5cm}|p{1.2 cm}|p{1.2 cm}|}
\hline 
AU &BP4D &BP4D+ \\ \hline 
1	&21.07	&9.54\\ \hline 
2	&17.04	&8.01\\ \hline 
4	&20.22	&0.67\\ \hline 
6	&46.10	&65.88\\ \hline 
7	&54.90	&3.46\\ \hline 
10	&59.39	&57.37\\ \hline 
12	&56.18	&59.99\\ \hline 
14	&46.60	&32.46\\ \hline 
15	&16.96	&12.96\\ \hline 
17	&34.37	&0.67\\ \hline 
23	&16.56	&2.35\\ \hline 
24	&15.16	&-\\ \hline
\end{tabular}
\centering
\caption{Percentage of AU labeled frames with occurrences in BP4D and BP4D+.}
\label{Distribution}
\end{table}

For binary classification, we conducted 4 experiments for each 3-fold and 10-fold: (1) training and testing on BP4D; (2) training and testing on BP4D+;  (3) training on BP4D and testing on BP4D+; and (4) training on BP4D+ and testing on BP4D. For our 3-class problem, we performed 2 experiments: (1) training and testing on BP4D; and (2) training and testing on BP4D+. For BP4D we detected 12 AUs, and 11 for BP4D+, as AU 24 did not occur in the labeled frames of this dataset. We refer the reader to Tables \ref{table:BinaryF1}, \ref{table:Cross Validation}, or \ref{table:3ClassResults} for the list of AUs detected for each dataset.

With this type of classification, especially with imbalanced data (Table \ref{Distribution}), F1 score can be a better indicator of performance compared to classification accuracy \cite{valstarFERA15}. Considering this, we calculated the frame-based F1 score as ($F1-frame=\frac{2RP}{R+P}$) where R is recall and P is precision. This approach is also consistent with related works, allowing us to compare our results.
